Measurement and correction of variations in interstellar dispersion in high-precision pulsar timing

Signals from radio pulsars show a wavelength-dependent delay due to dispersion in the interstellar plasma. At a typical observing wavelength, this delay can vary by tens of microseconds on five-year time scales, far in excess of signals of interest to pulsar timing arrays, such as that induced by a gravitational-wave background. Measurement of these delay variations is not only crucial for the detection of such signals, but also provides an unparallelled measurement of the turbulent interstellar plasma at au scales. In this paper we demonstrate that without consideration of wavelength- independent red-noise, 'simple' algorithms to correct for interstellar dispersion can attenuate signals of interest to pulsar timing arrays. We present a robust method for this correction, which we validate through simulations, and apply it to observations from the Parkes Pulsar Timing Array. Correction for dispersion variations comes at a cost of increased band-limited white noise. We discuss scheduling to minimise this additional noise, and factors, such as scintillation, that can exacerbate the problem. Comparison with scintillation measurements confirms previous results that the spectral exponent of electron density variations in the interstellar medium often appears steeper than expected. We also find a discrete change in dispersion measure of PSR J1603-7202 of ~2x10^{-3} cm^{-3}pc for about 250 days. We speculate that this has a similar origin to the 'extreme scattering events' seen in other sources. In addition, we find that four pulsars show a wavelength-dependent annual variation, indicating a persistent gradient of electron density on an au spatial scale, which has not been reported previously.

==> reply_to_referee <==
We thank the referee for the careful consideration of the paper.

>> 
>> Reviewer's Comments: Reviewer: Verbiest, Joris
>> 
>> Dear Dr. Keith et al.,
>> 
>> I have read your revised manuscript ("Measurement and correction of
>> variations in interstellar dispersion in high-precision pulsar timing") with
>> great interest and was glad to see an already good paper being improved even
>> further. I still have a few remaining comments (listed below) but since
>> there is nothing dramatic, I'll leave the judgement of whether to implement
>> or ignore these, up to you and need not see a revised version of your paper.
>> 
>> Note that one of your authors (Yardley) doesn't seem to be added in the
>> MNRAS system, though his name is in the article pdf.
>> 
>> I am sorry to point out one thing that struck me as being slightly
>> unprofessional. Last time, I pointed out that when talking about
>> gravitational waves, it was a bit unfortunate to give two references that
>> discuss the same type of GW, instead of having some variety. Instead of
>> changing one reference into another (as suggested), you added a third
>> reference. Interestingly, all three references are from the same
>> collaboration. This led me to do a little counting and so I discovered the
>> fascinating fact that, even though your paper is filled from top to bottom
>> with mentions of pulsar timing arrays and even though half of your
>> literature references are to PTA-related publications, all of these
>> publications are to your own, Parkes PTA. There is not a single reference to
>> either the European or North-American pulsar timing array. To some degree
>> this is defensible because the Parkes PTA has been leading the field for
>> quite some time, but particularly in Section 1 (where I already asked for a
>> revision because the Jenet et al. (2006) and Yardley et al. (2011) seemed a
>> weird choice of references), it seems unjustified to provide two references
>> to GWB limits, without mentioning either the most recent or the most
>> constraining effort(s). I really don't like promoting references as a
>> referee, but to include both Jenet and Yardley without even mentioning the
>> van Haasteren et al. (2011) limit, truly must be an oversight.

We have changed the Jenet reference to van Haasteren.


>> 
>> Right after Equation 4, you introduce the new factor \Delta. It may be
>> worthwhile spelling out the fact that this is just a factor defined for
>> convenience; and not an actual weighted least-squares solution (as it is
>> presented now).

Defined \Delta more clearly.

>> 
>> Halfway through the first column on page 3 (about half a paragraph after
>> Equation 10), the usage of "N" starts to become rather unclear (and it gets
>> worse as the paper continues). It may help to specify more clearly what the
>> subscripts mean. Specifically, you first introduce: " At each wavelength
>> \lambda_i we have a series of N_i error estimates \sigma_ij " so I imagine
>> N_i is the number of ToAs at a given observing wavelength lambda_i. I
>> further imagine the subscript 'j' identifies these different observations
>> and hence the mean \sigma_mi^2 on the next line must be a lambda-dependent
>> quantity. This would suggest that the $N$ on the following two lines ("the
>> same as if we had $N$ observations of equal variance...") really ought to be
>> $N_i$. A bit further, though, there is talk about "resampling each
>> wavelength with $N$ samples", suggesting that you don't just take the
>> average uncertainty, but average the measurements in some other fashion. I
>> presume this entire discussion is really not quite relevant because the real
>> data will probably be too inhomogeneous anyway (in many if not all cases),
>> so the discussion is mostly academic, but just because of that reason it
>> should be important to be clear about subscripts. In the next section,
>> moreover, you introduce $N_s$, which seems to be similar in nature to the
>> $N$ you just used, though the difference is not clearly defined. (N seems to
>> be the number of ToAs you end up with in each frequency band, after
>> averaging. N_s seems to be the number of DM measurements you have. I imagine
>> these would be identical?)

We have modified the text to make this clearer. Ni is the number of ToAs at
wavelength i, N is a conceptual value used to derive the white noise PSD. N_s
is the actual number of DM samples measured.

>> 
>> The update to Table 1 seems to have resulted in some important mismatches
>> with the text. In particular, P_w,TDM does not seem to appear in the table
>> anymore, even though it is stated in the text (page 3, left-hand column,
>> 6th-last line) that it is.

You are right that P_w,TDM was missing from Table 1. This has been added.

>> 
>> A small word on weighting. In my previous comments I pointed out that the DM
>> model the authors use, is unweighted, which is clearly sub-optimal. The
>> response was that the DM values were derived from a weighted fit and that
>> hence the DM(t) estimates were weighted as well. However, the point I was
>> making was that the linear interpolation of the DM values (which uses at
>> most two DM measurements at any point anyway) is inherently unweighted. To
>> me it intuitively makes more sense to use somewhat more data and use some
>> form of a weighted interpolation, instead of the very simplified linear,
>> unweighted scheme. Admittedly this doesn't matter as long as the DM
>> measurements are all of roughly equal quality which seems to be the case in
>> most of the PPTA data sets. For less uniform data sets this interpolation
>> may require a different approach, though.

It is very possible to use a more complex function for the DM correction.
However the linear interpolation is conservative. We recommend that other
analysts not use a more complex weighting unless they are confident that the
estimated uncertainties on their observations are quite accurate.  With linear
interpolation the effects of a poor uncertainty estimate cannot propagate far
from its epoch. Since the samples DM(t_i) are weighted averages, a weighted
interpolation will make little difference except, as the reviewer notes, in
cases where the sampling is highly irregular. Such cases can occur and should
be handled with caution.

>> 
>> The caption of Table 1 is not accurate anymore: it omits the fact that the
>> powers are now all expressed relative to that at 20cm. Also, it may be good
>> to explicitly specify that the "current observing strategy" is \alpha = 0.5.

Ok - done.


>> 
>> There is some inconsistency with the abbreviation for "year". Throughout
>> most of the paper, the standard "yr" is used, but towards the end of section
>> 3, in two instances "y" is used instead. (Also in the second paragraph of
>> section 4.1.)

Ok - fixed.

>> 
>> In the second paragraph of section 4, the parameter \sigma_o is used, but I
>> don't recall having seen that parameter before. Please specify what it is.

Changed to \sigma_ij, i.e. the ToA uncertainty.

>> 
>> It is unclear to me why the 90% confidence limits are plotted in Figure 1
>> and 2 (as opposed to the more traditional 68 or 95% limits).

90% confidence limits are chosen as one often wants to give a bounded limit to
the power spectrum, i.e. be 95% confident that the PSD is below some value.
The 95% confidence upper-limit is the same as the top of the 90% confidence
error bar, and the 95% lower-limit is the same as the bottom of the 90%
confidence error bar.

>> 
>> The authors have taken my comment about errors vs. uncertainties on board,
>> but not everywhere. In particular in the caption of Figure 3, it may be good
>> to replace "error" with "uncertainty".

Changed as suggested.

>> 
>> In Table 2, you present scintillation bandwidths and time scales. I presume
>> these were all scaled to some reference frequency, but this seems to be
>> unspecified, at least in the caption.

Changed caption to specify that these values are derived at 20cm.

>> 
>> Towards the end of Section 5.1, there is another reference to "P_w,TDM,
>> tabulated in Table 1", although it isn't tabulated there anymore.

Fixed as above.

>> 
>> At the start of Section 5.2, the statement that "one can see by eye that
>> there are statistically significant changes with time" is a bit frustrating.
>> I admit that in most cases I may agree with the statement, though one is
>> left wondering why we need to do this by eye. There either is statistical
>> significance (in which case it can be quantified), or there isn't (in which
>> case we don't want to 'eyeball' it).

Although it is appealing to imagine that the behaviour of a time series
described as a random process can be determined completely automatically, this
is not yet the case. In the paper we do use statistical tests to determine the
level of DM variations, however we feel that it is wise to consider the plots
subjectively as a starting point for understanding the data. Indeed, this is
why we have included this figure in the paper.

Nevertheless, there are statistically significant changes, and so we have
removed the "by eye" qualifier.

>> 
>> On a linguistic note, I would like to point out that the ISM is not a
>> (random) process, notwithstanding the author's claim in Section 5.2.

Ok - changed to "turbulent".

>> 
>> In the caption of Figure 5, you describe the dashed line as displaying the
>> "smoothed values". Is this dashed line actually derived from a smoothing of
>> the data, or from linear interpolation of data that were fitted over longer
>> intervals (i.e. did the same DM measurements result in the smoothed line, or
>> were there less frequent DM values to start with?)

Corrected to explain that this is the DM(t) derived from the fit using a longer
timescale.

>> 
>> Looking at Figure 6, I find it striking that the turnover in the structure
>> function of PSR J0437-4715 happens clearly above lags of 1000 days, even
>> though a subset of these authors have published an almost identical
>> structure function back in 2007 (You et al.), which showed the exact same
>> turnover, well below the 1000 day lag. Can this be explained?

The structure functions have very large uncertainties at large lags. These are
reflected in the dashed uncertainties shown on the figure (Note, an error was
discovered in the plotted dashed lines in the previous version which made this
harder to see. This has now been corrected). It is possible that this is a
"real" feature but it is currently not statistically significant.

>> 
>> Another thing I don't understand about Figure 6, is the smallest lags
>> displayed. The authors go through quite a bit of trouble to find the
>> shortest time scale on which DM variations are relevant. As far as I
>> understand, their final DM-determination intervals are tabulated in the
>> final column of Table 2. However, in Figure 6 there seems to be information
>> at even shorter time scales. For example, it is stated that the sample
>> interval T_s for PSR J1744-1134 is 1 year. However, its structure function
>> has a clear data point below 100 days lag. I presume this only looks like a
>> mismatch because of a gap in my understanding, but it would be good if such
>> misunderstandings could be avoided by explaining where these apparent
>> mismatches come from. (In other words: how can we have structure function
>> information below 100 days but only have useful DM information above 300
>> days?)

In fact we perform a preliminary analysis with the DM sampled at 0.25yr^-1, to
improve our estimate of the optimal sampling, because the extrapolation of
diffractive scintillation by 4 or 5 orders of magnitude can be quite uncertain.
We show the structure function with finer sampling than we ultimately use in DM
correcting the observations. The structure function flattens slowly as the
white noise limit is approached because we correct the structure function by
subtracting the white noise contribution. However, below the "corner time
scale" it is increasingly dominated by white noise.

>> 
>> Still on Figure 6, the caption tells us the "66%" confidence limits are
>> shown. Again I wonder why the more traditional 68% confidence limit wasn't
>> used instead.

Fixed to use 68% errors.


>> 
>> Finally on Figure 6, I'm not sure if the simulated 66% confidence regions
>> indicate "systematic errors" rather than "statistical uncertainties". (Note
>> this 66% is also referred to in the text of section 5.3.)

You are right that this isn't really a systematic error, but the uncertainty in
the estimation of the structure function of a Kolmogorov process caused by the
finite length of the observations. The caption has been updated to indicate
this.

>> 
>> Towards the end of Section 5.3, you state that 'y' or 'n' indicate "that we
>> believe that the DM correction is likely to improve the residuals." I hope
>> this is unfortunate wording, because frankly if you need to "believe" that a
>> method improves the results, then it is quite likely that it doesn't. I
>> wonder if evaluation of the chi-squared values in two cases -- firstly in
>> the determination of the DM model based on the DM measurements; and secondly
>> in the implementation of the DM model in the timing residuals -- might cast
>> some more light on the effectiveness and overall quality of the method, its
>> DM model and the application of said model. This clearly isn't crucial at
>> present, but maybe it's something to think about for any future work.

The uncertainty in knowing if the DM correction has improved the residuals is
due to the fact that in these pulsars the amplitude of the DM variations only
appears in the lowest spectral channels and so there are insufficient statistics
to determine if the correction has improved things. In the paper we try and be
conservative such that even though the spectrum may show less red noise, we
assume that this could entirely be due to the uncertainty in spectral
estimation. Even though the improvement is not statically significant in this
conservative estimation, we feel that it is useful to indicate that the pulsar
may have been improved as the DM correction will become more important with
time and it is likely that these pulsars will be next to show significant
improvement.

>> 
>> Comparing RMS values is -- as the authors know -- always a tricky thing to
>> do, although it certainly is interesting. One point that may do with some
>> extra clarification, is what the pre-RMS values were based on. Do these
>> numbers contain all ToAs from all frequency bands, or only the 20cm data?
>> Was the timing model fitted to all these frequency bands jointly, or only to
>> the 20cm data?

Text is updated to clarify that these are the RMS of the 20-cm data only. The
timing model was fit before spectral analysis in all cases.


>> 
>> Towards the end of page 12 (Section 7, 3/4 paragraphs), you need equal signs
>> in addition to the inequalities in 0<alpha<1.

Ok.

>> Also, a few lines lower down, you write: " We use t_o2 as the reference
>> because it usually has the highest S/N ratio " Sadly, I don't think t_o2 has
>> been defined. Assuming the authors have listed their frequencies in linear
>> order, we could derive that they mean the 20cm data, but frankly this isn't
>> clear at all, especially since the highest S/N ratio could be expected to
>> occur in the 50cm band instead.

Changed to reference the actual wavelength rather than the numerical index.

>> 
>> At the end of Section 7, you suggest that "broadband receivers reduce
>> difficulties of aligning pulse profiles [...] and therefore allows for more
>> accurate measurement of both the DM and the arrival time." I don't think
>> this is true. Whatever receiver one uses, there will always be an ambiguity
>> between the pulse shape evolution and the DM. Whether continuous frequency
>> coverage will improve the measurement of the arrival time seems doubtful and
>> unsubstantiated, but the fact that the DM will still be totally covariant
>> with the pulse profile evolution, seems beyond doubt.

It is true that the DM will still be covariant with the pulse profile
evolution.  We have modified the text to indicate that it is DM variations
rather than absolute DM that are better measured. We feel that it is true that
a wide-band system will reduce the systematic issues caused by observing with
different receivers over different days, and therefore improve the accuracy of
the DM correction.

>> 
>> In the end of Section 8, where you describe how modelling of the ISM is
>> possible and could enable more precise DM removal, I would encourage you to
>> mention some references. This paragraph is simply far too interesting and
>> far too non-committal to be satisfactory without reference.

Unfortunately we do not know of anyone that has attempted this to date.  We
have been successful with J0613-0200 and intend to continue this work with other
pulsars Certainly this is something that we hope to publish as soon as
possible.

>> 
>> Throughout the paper, you have alternatively talked about "DM variations" or
>> "variation in DM" -- sometimes in singular, sometimes in plural. While the
>> plural form is the more common one (according to me), it is a bit disturbing
>> that the plurality changes almost continuously, in this paper.

We have replaced variation with variations wherever appropriate.

>> 
>> In appendix A, you describe E as a column vector of uncertainties. In this
>> case, I would hope it's either a column vector of errors or a column vector
>> of white noise contributions. These are indeed quantified by uncertainties,
>> but they are not the same. The uncertainties describe the white noise
>> process of which the elements of vector E are single realisations.
>> 

Ok - changed to errors.

